Expanding Label Sets for Graph Convolutional Networks

In recent years, Graph Convolutional Networks (GCNs) and their variants have been widely utilized in learning tasks that involve graphs. These tasks include recommendation systems, node classification, among many others. In node classification problem, the input is a graph in which the edges represent the association between pairs of nodes, multi-dimensional feature vectors are associated with the nodes, and some of the nodes in the graph have known labels. The objective is to predict the labels of the nodes that are not labeled, using the nodes features, in conjunction with graph topology. While GCNs have been successfully applied to this problem, the caveats that they inherit from traditional deep learning models pose significant challenges to broad utilization of GCNs in node classification. One such caveat is that training a GCN requires a large number of labeled training instances, which is often not the case in realistic settings. To remedy this requirement, state-of-the-art methods leverage network diffusion-based approaches to propagate labels across the network before training GCNs. However, these approaches ignore the tendency of the network diffusion methods in biasing proximity with centrality, resulting in the propagation of labels to the nodes that are well-connected in the graph. To address this problem, here we present an alternate approach to extrapolating node labels in GCNs in the following three steps: (i) clustering of the network to identify communities, (ii) use of network diffusion algorithms to quantify the proximity of each node to the communities, thereby obtaining a low-dimensional topological profile for each node, (iii) comparing these topological profiles to identify nodes that are most similar to the labeled nodes.

==> MainFig <==
\begin{picture}(0,0)%
\includegraphics{MainFig}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3113,1250)(814,-1286)
\end{picture}%


==> RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
GCNs have received significant attention over the past few years, since they effectively integrate node features and graph structure for many graph learning tasks~\cite{Kipf}. 
Most of the work in recent years focuses on addressing the caveats of GCNs that are inherited from classical deep neural networks.
%which derive primary inspiration for the development of GCNs, have been tried to addressed to more effectively use GCNs in broad range of applications. 
One of the limitations coming from deep learning is that training neural networks can be computationally very expensive for real-world large graphs~\cite{klicpera2018combining}. 
To circumvent computational complexity of training,  Klicpera {\em et al.} propose using personalized random walk before training the neural networks. 
This approach is further extended by Wu {\em et al.}~\cite{FWu} who simplify GCNs using a linear transformation, which is also similar to to algebraic formulation of random walks.

Another line of research aims to address the issues caused by the limited availability of labeled data~\cite{AAAI18Li}. To alleviate this problem, Li and et al.~\cite{AAAI18Li} propose to expand the set of labeled nodes using a random walk based approach. In particular, they use ParWalk~\cite{WuX} in a way that is similar to the use of personalized page rank~\cite{AAAI18Li}, by taking proxmity and connectivity of into account to take advantage of the assortativity of the labels in the graph.

In this paper, we also focus on expanding the label set to address the 
limited labeled samples problem. 
Our method is fundamentally different from existing approaches in that it exploits the intrinsic topological information of nodes to incorporate assortativity without bias from other factors, such as the individual connectivity of the nodes~\cite{AAAI18Li}.
Our method can be used to efficiently and accurately classifying unknown node labels in the context of node classification with GCNs. 




